Improving information retrieval from electronic health records using dynamic and multi-collaborative filtering

Due to the rapid growth of information available about individual patients, most physicians suffer from information overload when they review patient information in health information technology systems. In this manuscript, we present a novel hybrid dynamic and multi-collaborative filtering method to improve information retrieval from electronic health records. This method recommends relevant information from electronic health records for physicians during patient visits. It models information search dynamics using a Markov model. It also leverages the key idea of collaborative filtering, originating from Recommender Systems, to prioritize information based on various similarities among physicians, patients and information items. We tested this new method using real electronic health record data from the Indiana Network for Patient Care. Our experimental results demonstrated that for 46.7% of testing cases, this new method is able to correctly prioritize relevant information among top-5 recommendations that physicians are truly interested in.

==> graphs/LOOV_graph.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3566,154){\makebox(0,0){\strut{}Time}}%
      \csname LTb\endcsname%
      \put(5816,4602){\makebox(0,0)[r]{\strut{}training part}}%
      \csname LTb\endcsname%
      \put(5816,4382){\makebox(0,0)[r]{\strut{}training term}}%
      \csname LTb\endcsname%
      \put(5816,4162){\makebox(0,0)[r]{\strut{}evaluation term}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{LOOV_graph}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/pat_similarity_hist2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,1312){\makebox(0,0)[r]{\strut{}$1\times10^{8}$}}%
      \put(1078,1919){\makebox(0,0)[r]{\strut{}$2\times10^{8}$}}%
      \put(1078,2527){\makebox(0,0)[r]{\strut{}$3\times10^{8}$}}%
      \put(1078,3134){\makebox(0,0)[r]{\strut{}$4\times10^{8}$}}%
      \put(1078,3742){\makebox(0,0)[r]{\strut{}$5\times10^{8}$}}%
      \put(1078,4350){\makebox(0,0)[r]{\strut{}$6\times10^{8}$}}%
      \put(1210,484){\makebox(0,0){\strut{}$0$}}%
      \put(1769,484){\makebox(0,0){\strut{}$0.1$}}%
      \put(2329,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(2888,484){\makebox(0,0){\strut{}$0.3$}}%
      \put(3447,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(4007,484){\makebox(0,0){\strut{}$0.5$}}%
      \put(4566,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(5125,484){\makebox(0,0){\strut{}$0.7$}}%
      \put(5684,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(6244,484){\makebox(0,0){\strut{}$0.9$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Frequency}}}%
      \put(4006,154){\makebox(0,0){\strut{}Patient-Patient Similarity}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{pat_similarity_hist2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/pat_similarity_hist_0626.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1254,588){\makebox(0,0)[r]{\strut{}0.0005\%}}%
      \put(1254,873){\makebox(0,0)[r]{\strut{}0.001\%}}%
      \put(1254,1822){\makebox(0,0)[r]{\strut{}0.01\%}}%
      \put(1254,2770){\makebox(0,0)[r]{\strut{}0.1\%}}%
      \put(1254,3719){\makebox(0,0)[r]{\strut{}1\%}}%
      \put(1254,4667){\makebox(0,0)[r]{\strut{}10\%}}%
      \put(1490,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.0}}}%
      \put(2011,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.1}}}%
      \put(2532,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.2}}}%
      \put(3053,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.3}}}%
      \put(3574,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.4}}}%
      \put(4095,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.5}}}%
      \put(4615,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.6}}}%
      \put(5136,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.7}}}%
      \put(5657,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.8}}}%
      \put(6178,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.9}}}%
      \put(6699,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1.0}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(352,2681){\rotatebox{-270}{\makebox(0,0){\strut{}non-zero frequency ($\log$)}}}%
      \put(4094,154){\makebox(0,0){\strut{}\simP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{pat_similarity_hist_0626}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/pat_similarity_hist_0718.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1122,588){\makebox(0,0)[r]{\strut{}0.001\%}}%
      \put(1122,1606){\makebox(0,0)[r]{\strut{}0.01\%}}%
      \put(1122,2624){\makebox(0,0)[r]{\strut{}0.1\%}}%
      \put(1122,3641){\makebox(0,0)[r]{\strut{}1\%}}%
      \put(1122,4659){\makebox(0,0)[r]{\strut{}10\%}}%
      \put(1361,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.0}}}%
      \put(1894,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.1}}}%
      \put(2428,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.2}}}%
      \put(2961,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.3}}}%
      \put(3495,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.4}}}%
      \put(4029,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.5}}}%
      \put(4562,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.6}}}%
      \put(5096,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.7}}}%
      \put(5629,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.8}}}%
      \put(6163,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.9}}}%
      \put(6696,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1.0}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(352,2681){\rotatebox{-270}{\makebox(0,0){\strut{}non-zero frequency ($\log$)}}}%
      \put(4028,154){\makebox(0,0){\strut{}\simP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{pat_similarity_hist_0718}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/pat_similarity_hist_0903.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1122,588){\makebox(0,0)[r]{\strut{}0.001\%}}%
      \put(1122,1606){\makebox(0,0)[r]{\strut{}0.01\%}}%
      \put(1122,2624){\makebox(0,0)[r]{\strut{}0.1\%}}%
      \put(1122,3641){\makebox(0,0)[r]{\strut{}1\%}}%
      \put(1122,4659){\makebox(0,0)[r]{\strut{}10\%}}%
      \put(1361,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.0}}}%
      \put(1894,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.1}}}%
      \put(2428,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.2}}}%
      \put(2961,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.3}}}%
      \put(3495,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.4}}}%
      \put(4029,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.5}}}%
      \put(4562,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.6}}}%
      \put(5096,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.7}}}%
      \put(5629,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.8}}}%
      \put(6163,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}0.9}}}%
      \put(6696,456){\rotatebox{-45}{\makebox(0,0)[l]{\strut{}1.0}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(352,2681){\rotatebox{-270}{\makebox(0,0){\strut{}non-zero frequency ($\log$)}}}%
      \put(4028,154){\makebox(0,0){\strut{}\simP}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{pat_similarity_hist_0903}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/phy_similarity_hist2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,1137){\makebox(0,0)[r]{\strut{}$1\times10^{6}$}}%
      \put(1078,1570){\makebox(0,0)[r]{\strut{}$2\times10^{6}$}}%
      \put(1078,2003){\makebox(0,0)[r]{\strut{}$3\times10^{6}$}}%
      \put(1078,2436){\makebox(0,0)[r]{\strut{}$4\times10^{6}$}}%
      \put(1078,2869){\makebox(0,0)[r]{\strut{}$5\times10^{6}$}}%
      \put(1078,3303){\makebox(0,0)[r]{\strut{}$6\times10^{6}$}}%
      \put(1078,3736){\makebox(0,0)[r]{\strut{}$7\times10^{6}$}}%
      \put(1078,4169){\makebox(0,0)[r]{\strut{}$8\times10^{6}$}}%
      \put(1078,4602){\makebox(0,0)[r]{\strut{}$9\times10^{6}$}}%
      \put(1210,484){\makebox(0,0){\strut{}$0$}}%
      \put(1769,484){\makebox(0,0){\strut{}$0.1$}}%
      \put(2329,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(2888,484){\makebox(0,0){\strut{}$0.3$}}%
      \put(3447,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(4007,484){\makebox(0,0){\strut{}$0.5$}}%
      \put(4566,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(5125,484){\makebox(0,0){\strut{}$0.7$}}%
      \put(5684,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(6244,484){\makebox(0,0){\strut{}$0.9$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Frequency}}}%
      \put(4006,154){\makebox(0,0){\strut{}Physician-Physician Similarity}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{phy_similarity_hist2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> graphs/term_similarity_hist2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(1078,1128){\makebox(0,0)[r]{\strut{}$1\times10^{7}$}}%
      \put(1078,1552){\makebox(0,0)[r]{\strut{}$2\times10^{7}$}}%
      \put(1078,1976){\makebox(0,0)[r]{\strut{}$3\times10^{7}$}}%
      \put(1078,2400){\makebox(0,0)[r]{\strut{}$4\times10^{7}$}}%
      \put(1078,2824){\makebox(0,0)[r]{\strut{}$5\times10^{7}$}}%
      \put(1078,3248){\makebox(0,0)[r]{\strut{}$6\times10^{7}$}}%
      \put(1078,3672){\makebox(0,0)[r]{\strut{}$7\times10^{7}$}}%
      \put(1078,4097){\makebox(0,0)[r]{\strut{}$8\times10^{7}$}}%
      \put(1078,4521){\makebox(0,0)[r]{\strut{}$9\times10^{7}$}}%
      \put(1210,484){\makebox(0,0){\strut{}$0$}}%
      \put(1769,484){\makebox(0,0){\strut{}$0.1$}}%
      \put(2329,484){\makebox(0,0){\strut{}$0.2$}}%
      \put(2888,484){\makebox(0,0){\strut{}$0.3$}}%
      \put(3447,484){\makebox(0,0){\strut{}$0.4$}}%
      \put(4007,484){\makebox(0,0){\strut{}$0.5$}}%
      \put(4566,484){\makebox(0,0){\strut{}$0.6$}}%
      \put(5125,484){\makebox(0,0){\strut{}$0.7$}}%
      \put(5684,484){\makebox(0,0){\strut{}$0.8$}}%
      \put(6244,484){\makebox(0,0){\strut{}$0.9$}}%
      \put(6803,484){\makebox(0,0){\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Frequency}}}%
      \put(4006,154){\makebox(0,0){\strut{}Term-Term Similarity}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{term_similarity_hist2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> markov_method.tex <==
The prediction scores of the first-order markov chain are obtained by using the transition probability matrix MC\_P as follows,
\begin{equation}
	\Sdyn(\physician,\patient,\term) = \text{MC\_P}(\term_l,\term),
\end{equation}
where $\term_l$ is the last search term of physician and patient $(\physician,\patient)$'s search sequence, $\term$ is a possible search term and
MC\_P is the transition probability of the first-order markov chain model.

The transition probability matrix has size of $|\text{T}|\times|\text{T}|$, where $\text{T}$ is the set of all search terms.
In the transition probability matrix MC\_P, the element $\text{MC\_P}(\term_1,\term_2)$ represents the probability of transition from term $\term_1$ to term $\term_2$.
In order to calculate the transition probability matrix, we need to calculate the transition frquency matrix MC\_F.
The element $\text{MC\_F}(\term_1,\term_2)$ is the frequency of transition from term $\term_1$ to 
term $\term_2$ in the training data as follows,
\begin{equation}
	\text{MC\_F}(\term_1,\term_2) = \text{C}(\term_1\to \term_2).
\end{equation}
Multiple search sequences of physician and patient pairs will be used as the training data of the first-order markov chain.
The transition probability matrix is obtained by normalizing each row of the transition frequency matrix as follows,
\begin{equation}
	\text{MC\_P}(\term_1, :) = \frac{\text{MC\_F}(\term_1,:)}{\sum_{\term}\text{MC\_F}(\term_1,\term)}
\end{equation}
where $\text{MC\_P}(\term_1, :)$ is the row of term $\term_1$ in transition probability matrix MC\_P and $\text{MC\_F}(\term_1,:)$
is the row of term $\term_1$ in transition frequency matrix MC\_F.


==> performance/paramter_study/additional_experiment/alpha_addi.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1286){\makebox(0,0)[r]{\strut{}0.20}}%
      \put(946,1867){\makebox(0,0)[r]{\strut{}0.25}}%
      \put(946,2449){\makebox(0,0)[r]{\strut{}0.30}}%
      \put(946,3030){\makebox(0,0)[r]{\strut{}0.35}}%
      \put(946,3612){\makebox(0,0)[r]{\strut{}0.40}}%
      \put(946,4193){\makebox(0,0)[r]{\strut{}0.45}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{}0.50}}%
      \put(1078,484){\makebox(0,0){\strut{}0}}%
      \put(1651,484){\makebox(0,0){\strut{}0.02}}%
      \put(2223,484){\makebox(0,0){\strut{}0.04}}%
      \put(2796,484){\makebox(0,0){\strut{}0.06}}%
      \put(3368,484){\makebox(0,0){\strut{}0.08}}%
      \put(3941,484){\makebox(0,0){\strut{}0.1}}%
      \put(4513,484){\makebox(0,0){\strut{}0.12}}%
      \put(5086,484){\makebox(0,0){\strut{}0.14}}%
      \put(5658,484){\makebox(0,0){\strut{}0.16}}%
      \put(6231,484){\makebox(0,0){\strut{}0.18}}%
      \put(6803,484){\makebox(0,0){\strut{}0.2}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}HR@N}}}%
      \put(3940,154){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3050,1097){\makebox(0,0)[r]{\strut{}HR@1}}%
      \csname LTb\endcsname%
      \put(3050,877){\makebox(0,0)[r]{\strut{}HR@2}}%
      \csname LTb\endcsname%
      \put(4433,1097){\makebox(0,0)[r]{\strut{}HR@3}}%
      \csname LTb\endcsname%
      \put(4433,877){\makebox(0,0)[r]{\strut{}HR@4}}%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}HR@5}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{alpha_addi}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> performance/paramter_study/alpha.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolorfalse
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(946,1286){\makebox(0,0)[r]{\strut{}0.20}}%
      \put(946,1867){\makebox(0,0)[r]{\strut{}0.25}}%
      \put(946,2449){\makebox(0,0)[r]{\strut{}0.30}}%
      \put(946,3030){\makebox(0,0)[r]{\strut{}0.35}}%
      \put(946,3612){\makebox(0,0)[r]{\strut{}0.40}}%
      \put(946,4193){\makebox(0,0)[r]{\strut{}0.45}}%
      \put(946,4775){\makebox(0,0)[r]{\strut{}0.50}}%
      \put(1078,484){\makebox(0,0){\strut{}0.0}}%
      \put(1651,484){\makebox(0,0){\strut{}0.1}}%
      \put(2223,484){\makebox(0,0){\strut{}0.2}}%
      \put(2796,484){\makebox(0,0){\strut{}0.3}}%
      \put(3368,484){\makebox(0,0){\strut{}0.4}}%
      \put(3941,484){\makebox(0,0){\strut{}0.5}}%
      \put(4513,484){\makebox(0,0){\strut{}0.6}}%
      \put(5086,484){\makebox(0,0){\strut{}0.7}}%
      \put(5658,484){\makebox(0,0){\strut{}0.8}}%
      \put(6231,484){\makebox(0,0){\strut{}0.9}}%
      \put(6803,484){\makebox(0,0){\strut{}1.0}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}HR@N}}}%
      \put(3940,154){\makebox(0,0){\strut{}$\alpha$}}%
      \csname LTb\endcsname%
      \put(3050,1097){\makebox(0,0)[r]{\strut{}HR@1}}%
      \csname LTb\endcsname%
      \put(3050,877){\makebox(0,0)[r]{\strut{}HR@2}}%
      \csname LTb\endcsname%
      \put(4433,1097){\makebox(0,0)[r]{\strut{}HR@3}}%
      \csname LTb\endcsname%
      \put(4433,877){\makebox(0,0)[r]{\strut{}HR@4}}%
      \csname LTb\endcsname%
      \put(5816,1097){\makebox(0,0)[r]{\strut{}HR@5}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{alpha}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> tables/dataset_small.tex <==
\begin{table}[!h] 
  \centering
  \caption{Statistics of INPC Dataset}
  \label{tbl:dataset}
  \begin{small}
  \begin{threeparttable}
    \begin{tabular}{
	@{\hspace{0pt}}l@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{10pt}}
        @{\hspace{10pt}}r@{\hspace{0pt}}
        %@{\hspace{7pt}}r@{\hspace{0pt}}
        %@{\hspace{7pt}}r@{\hspace{5pt}}
      }
      \toprule
      dataset   &  \#\patient  & \#\physician & \#\term & \#\seq &
      len(\seq) \\%& len(\seq)/\#\patient  & len(\seq)/\#\seq \\
      \midrule
      INCP               & 13,819 & 2,121 & 9,781 & 24,183 & 69,770 \\%& 5.049 & 2.885 \\
      training &  8,471 & 1,542 & 6,550 & 13,677 & 38,553 \\%& 4.551 & 2.819 \\ 
      testing  &   624  & 147   &   654 &    692 &  2,506 \\%& 4.016 & 3.621 \\
      \bottomrule
    \end{tabular}
    \begin{tablenotes}
      \setlength\labelsep{0pt}
      \begin{footnotesize}
      \item
	In this table, \#\patient is the number of patients;
        \#\physician is the number of physicians;
        \#\term is the number of terms;
        \#\seq is the number of sequences;
        len(\seq) is total length of sequences. 
%        len(\seq)/\#\patient is average length of sequences per patient
%        and len(\seq)/\#\seq is average length of sequences. 
        \par
      \end{footnotesize}
    \end{tablenotes}
  \end{threeparttable}
  \end{small}
\end{table}


==> tables/overall_cutoffdate_backup.tex <==
%\begin{table*}[t!]
  \centering
  %\tbl{\mbox{Performance on Ranking New Drugs}}
  \caption{\mbox{Overall Performance Table in \cutoff}}
  {
  \label{tbl:results:overal_perf_table}
  %  \vspace{-10pt}
  \begin{small}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{0pt}}c@{\hspace{0pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}          
        }        
        %        \hline\hline
        \toprule%\toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{5}{c}{performance} \\
        %        \cline{1-14}
        \midrule
        \multirow{2}{*}{\foMC}
        & \multicolumn{6}{c}{-}	& \small{HR@$1$} & \small{HR@$2$}  & \small{HR@$3$}  & \small{HR@$4$}   & \small{HR@$5$}\\

	\cmidrule(r){2-12}
	& \multicolumn{6}{c}{-} & 0.20187         & 0.29720           & 0.33832           & 0.37757            & 0.39252\\

        \cmidrule(r){1-12}
	\multirow{6}{*}{\ypCF}
          & Identification  & \physician\_self\_ref & \patient\_self\_ref & \#sim\_phy & \multicolumn{2}{c}{\#sim\_pat}  & \small{HR@$1$}  & \small{HR@$2$} & \small{HR@$3$}  & \small{HR@$4$}               & \small{HR@$5$}    \\
        \cmidrule(r){2-12}
	& \simPY            & Yes                   & No                  & 1          & \multicolumn{2}{c}{100}         & 0.22430           & 0.32336          & 0.36822           & 0.37757                        & 0.38692\\
	& \simPY	    & Yes		    & Yes		  & 


	%\hline
        \cmidrule(r){1-12}
        

        \multirow{2}{*}{\TptCF}
        & \multicolumn{3}{c}{\#sim\_pats}  &  \multicolumn{3}{c}{term\_sim\_threshold}  & \small{HR@$1$} & \small{HR@$2$}  & \small{HR@$3$}  & \small{HR@$4$} & \small{HR@$5$} \\
        \cmidrule(r){2-12} 
        % 
	& \multicolumn{3}{c}{160}        &  \multicolumn{3}{c}{0.1}                   & 0.213          & 0.279           & 0.303           & 0.322          & 0.331\\
                                                                                                                                                    

	%
        \cmidrule(r){1-12}
        \multirow{2}{*}{\method\_\ypCF}
	& Identification  & \physician\_self\_ref & \patient\_self\_ref & \#sim\_phy & \#sim\_pat & $\alpha$  & \small{HR@$1$}  & \small{HR@$2$} & \small{HR@$3$}  & \small{HR@$4$}  & \small{HR@$5$}    \\

        \cmidrule(r){2-12}
	& \simYP          & No                    & No                  & 1        & 1            & 0.2       & 0.243           & 0.314          & 0.353           & 0.398           & 0.422\\

	\cmidrule(r){1-12}
	\multirow{2}{*}{\method\_\TptCF}
	& \multicolumn{3}{c}{\#sim\_pats}  &  \multicolumn{2}{c}{term\_sim\_threshold} & $\alpha$  & \small{HR@$1$} & \small{HR@$2$}  & \small{HR@$3$}  & \small{HR@$4$} & \small{HR@$5$} \\
	\cmidrule(r){2-12}
	& \multicolumn{3}{c}{60}        &  \multicolumn{2}{c}{0.4}                  & 0.8         & 0.228          & 0.307           & 0.335           & 0.359          & 0.379\\
        \bottomrule%\bottomrule
%      \hline\hline
      \end{tabular}
\begin{comment}
      \begin{tablenotes}
       \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item 
          \par
        \end{scriptsize}
      \end{tablenotes}
\end{comment}
  \end{threeparttable}
  \end{small}
  } %end tbl
\vspace{-10pt}
\end{table*}



==> tables/overall_cutoffdate_small.tex <==
\begin{table}[t!]
  \centering
  %\tbl{\mbox{Performance on Ranking New Drugs}}
  \caption{\mbox{Overall Performance Comparison}} % with \cutoff (08/15/2013)}}
  {
  \label{tbl:results:cuttof:0815}
  %  \vspace{-10pt}
  \begin{small}
  \begin{threeparttable}
      \begin{tabular}{
	@{\hspace{7pt}}c@{\hspace{7pt}}
        %        
        %@{\hspace{7pt}}c@{\hspace{7pt}}
        %@{\hspace{7pt}}r@{\hspace{7pt}}
        %@{\hspace{7pt}}r@{\hspace{7pt}}
        %@{\hspace{7pt}}r@{\hspace{7pt}}
        %@{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        }        
        %        \hline\hline
        \toprule%\toprule
        method   %& sim & $\alpha$ & $|\Sp|$ & $|\Sy|$ & $\beta$ &
        & HR@1 & HR@2 & HR@3 & HR@4 & HR@5 \\
        %        \cline{1-14}
        \midrule
        \multirow{3}{*}{\method-\ypCF}  %& \multirow{3}{*}{\simPY} %& $ 0.2$  & $   1$ & $   1$ & - &
        & \textbf{0.247} & 0.357 & \ul{\textbf{0.426}}  &  \ul{\textbf{0.441}} & 0.464 \\
        %&                         %& $ 0.5$  & $   1$ & $   1$ & - &
        & 0.245 & \ul{\textbf{0.363}} & 0.422  &  0.439 & 0.464 \\
        %&                         %& $ 0.2$  & $ 100$ & $   2$ & - &
        & 0.226 & 0.351 & 0.404  &  0.430 & \ul{\textbf{0.467}} \\
        %\cmidrule(r){2-12}
        %& \multirow{5}{*}{\simYP} %& $ 0.5$  & $   3$ & $   5$ & - &
        %& \textbf{0.254} & 0.329 &  0.353  &  0.379 & 0.426 \\
        %&                         %& $ 0.1$  & $   3$ & $   2$ & - &
        %& 0.230 & \textbf{0.346} & 0.366 &  0.402 & 0.432 \\
        %&                         %& $ 0.1$  & $   1$ & $  20$ & - &
        %& 0.230 & 0.331 & \textbf{0.391} &  0.424 & 0.447 \\
        %&                         %& $ 0.1$  & $   1$ & $   1$ & - &
        %& 0.222 & 0.331 & 0.383 &  \textbf{0.430} & 0.447 \\
        %&                         %& $ 0.2$  & $   1$ & $   1$ & - &
        %& 0.222 & 0.323 & 0.378 &  0.426 & \textbf{0.449} \\

        \midrule
        \multirow{5}{*}{\method-\TptCF}  %& - & $0.8$  &$  60$ & - & $ 0.4$ &
        & \textbf{0.228} & 0.307 & 0.335 & 0.359 & 0.379\\
        %& - & $0.7$  &$  40$ & - & $ 0.1$ &
        & 0.213 & \textbf{0.312} & 0.348 & 0.376 & 0.398\\
        %& - & $0.8$  &$ 200$ & - & $ 0.1$ &
        & 0.213 & 0.303 & \textbf{0.353} & 0.376 & 0.400\\
        %& - & $0.6$  &$   5$ & -
        %& $ 0.1$ &
        & 0.209 & 0.297 & 0.344 & \textbf{0.383} & 0.406\\
        %& - & $0.1$  &$   1$ & -
        %& $ 0.1$ &
        & 0.200 & 0.310 & 0.346 & 0.381 & \textbf{0.413}\\

        \bottomrule%\bottomrule
%      \hline\hline
      \end{tabular}
      \begin{tablenotes}
       \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item %In this table, %the column ``sim'' corresponds to similarity identification
          %methods; $\alpha$ is the weight on CF component in \method;
          %$|\Sp|$ is the number of similar patients; $|\Sy|$ is the number of similar
          %physicians; $\beta$ is the similarity threshold to identify similar terms.
          %
          The best performance of each method under each metric is \textbf{bold}.
          The best overall performance of all methods under each metric is
          \underline{\textbf{underlined}}. 
          \par
        \end{scriptsize}
      \end{tablenotes}
  \end{threeparttable}
  \end{small}
  } %end tbl
  %\vspace{-10pt}
\end{table}




==> tables/overall_loo.tex <==
\begin{table}[h!]
  \begin{center}
  %\tbl{\mbox{Performance on Ranking New Drugs}}
  \caption{\mbox{Overall Performance Comparison with \loocv}}
%  {
  \label{tbl:results:loocv}
  %  \vspace{-8pt}
%  \begin{small}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{7pt}}c@{\hspace{7pt}}
        %        
        @{\hspace{7pt}}c@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{0pt}}r@{\hspace{0pt}}
        %
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}
        @{\hspace{7pt}}r@{\hspace{7pt}}          
        }        
        \toprule
	method   & sim & $\alpha$ & $|\Sp|$ & $|\Sy|$ & $\beta$ & & HR@1 & HR@2 & HR@3 & HR@4 & HR@5 \\
        \midrule
        \foMC                     & -                       & -          & - & - & - & & \ul{\textbf{0.328}} & \textbf{0.419} & \textbf{0.457} & \textbf{0.482} & \textbf{0.505}\\

        \midrule
        \multirow{5}{*}{\ypCF}    & \multirow{2}{*}{\simPY} &- & $ 100$ & $   1$  &- & & \textbf{0.212} & \textbf{0.282} &         0.308  &          0.327 &          0.342 \\
                                  &                         &- & $ 100$ & $   2$  &- & &        0.196   &         0.275  & \textbf{0.310} & \textbf{0.334} & \textbf{0.353} \\
                                  \cmidrule(r){2-12}
                                  & \multirow{3}{*}{\simYP} &- & $   1$ & $ 100$  &- & & \textbf{0.206} & 0.233 &  0.240   &  0.242 &   0.244 \\
                                  &                         &- & $   2$ & $ 100$  &- & & 0.202 & \textbf{0.242} &  0.262   &  0.270 &   0.274 \\
                                  &                         &- & $   4$ & $ 100$  &- & & 0.181 & 0.233 &  \textbf{0.268}   &  \textbf{0.284} &   \textbf{0.296} \\
%                                 &                         &- & $   5$ & $ 100$  &- & & 0.175 & 0.227 &  0.262   &  0.283 &   \textbf{0.296} \\

        \midrule
        %
        \multirow{3}{*}{\TptCF}   &- &- &$ 2,200$ &- & $ 1.0$ & & \textbf{0.285} & \textbf{0.373} & 0.401 & 0.421 & 0.435\\
                                  &- &- &$ 2,600$ &- & $ 0.6$ & & 0.283 & 0.372 & \textbf{0.402} & 0.422 & 0.437\\
                                  &- &- &$ 2,000$ &- & $ 0.3$ & & 0.277 & 0.366 & 0.399 & \textbf{0.424} & \textbf{0.438}\\
%                                 &- &- &$ 2,600$ &- & $ 0.6$ & & 0.277 & 0.366 & 0.399 & 0.423 & \textbf{0.438}\\
        \midrule
        %
        \multirow{3}{*}{\method-\ypCF} & \multirow{1}{*}{\simPY} & $0.1$  & $ 100$ & $ 1$ &- & & \textbf{0.248} & \textbf{0.371} &  \textbf{0.429}  &  \textbf{0.469} & \textbf{0.499}\\
                                       \cmidrule(r){2-12}
                                       & \multirow{3}{*}{\simYP} & $0.1$  & $   1$ & $ 1$ &- & & \textbf{0.306} & \textbf{0.407} &         0.451  &          0.478 &          0.501 \\
%                                      &                         & $0.1$  & $   2$ & $ 1$ &- & & 0.304 & \textbf{0.407} &         0.450  &          0.478 &          0.502 \\
                                       &                         & $0.1$  & $ 100$ & $ 1$ &- & & 0.304 & 0.405  &    \textbf{0.452}    &          \textbf{0.483} & \textbf{0.509} \\
        \midrule
        %
 %       \multirow{3}{*}{\method-\TptCF} &- &$0.1$  &$ 1$ &- & $ 0.3$ & & \ul{\textbf{0.328}} & 0.422 & \ul{\textbf{0.460}} & 0.486 & 0.508\\
        \multirow{2}{*}{\method-\TptCF} &- &$0.1$  &$ 1$ &- & $ 0.1$ & & \ul{\textbf{0.328}} & \ul{\textbf{0.423}} & \ul{\textbf{0.460}} & \ul{\textbf{0.488}} & 0.509\\
                                        &- &$0.1$  &$ 5$ &- & $ 0.1$ & & 0.325 & 0.421 & \ul{\textbf{0.460}} & 0.487 & \ul{\textbf{0.510}}\\
        \bottomrule
      \end{tabular}
  \end{threeparttable}
  \begin{tablenotes}
%    \setlength\labelsep{0pt}
    \begin{footnotesize}
    \item
      \textcolor{red}{not aligned well?}
      The best performance under each metric for each method is \textbf{bold}.
      The best performance under each metric over all the methods is \ul{underlined}. \par
    \end{footnotesize}
  \end{tablenotes}
%  \end{small}
%  } %end tbl
%\vspace{-10pt}
  \end{center}
\end{table}



==> tables/overall_loo_backup.tex <==
\begin{table*}[t!]
  \centering
  %\tbl{\mbox{Performance on Ranking New Drugs}}
  \caption{\mbox{Overall Performance Table in \loocv}}
  {
  \label{tbl:results:overal_perf_table}
  %  \vspace{-10pt}
  \begin{small}
  \begin{threeparttable}
      \begin{tabular}{
        @{\hspace{5pt}}c@{\hspace{5pt}}
        @{\hspace{0pt}}c@{\hspace{0pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}
        @{\hspace{5pt}}r@{\hspace{5pt}}          
        }        
        %        \hline\hline
        \toprule%\toprule
        method   & \multicolumn{6}{c}{parameters} & \multicolumn{5}{c}{performance} \\
        %        \cline{1-14}
        \midrule
        \multirow{2}{*}{\foMC}
        & \multicolumn{6}{c}{-}	& \small{HR@$1$} & \small{HR@$2$}  & \small{HR@$3$}  & \small{HR@$4$}   & \small{HR@$5$}\\

	\cmidrule(r){2-12}
	& \multicolumn{6}{c}{-} & 0.32767        & 0.41905         & 0.45699         & 0.48248          & 0.50514\\

        \cmidrule(r){1-12}
	\multirow{6}{*}{\ypCF}
          & Identification  & \physician\_self\_ref & \patient\_self\_ref & \#sim\_phy & \multicolumn{2}{c}{\#sim\_pat}  & \small{HR@$1$}  & \small{HR@$2$} & \small{HR@$3$}  & \small{HR@$4$}               & \small{HR@$5$}    \\
        \cmidrule(r){2-12}
	& \simPY            & Yes                   & No                  & 1          & \multicolumn{2}{c}{100}         & 0.21161           & 0.28175          & 0.30777           & 0.32737                        & 0.34176\\
	& \simPY            & Yes                   & No                  & 1          & \multicolumn{2}{c}{100}         & 0.21161           & 0.28175          & 0.30777           & 0.32737                        & 0.34176\\
	& \simPY	    & Yes		    & No		  & 2	       & \multicolumn{2}{c}{100}	 & 0.19559	     & 0.27549	        & 0.31023           & 0.33378			     & 0.35264\\
	& \simPY	    & Yes		    & No		  & 2	       & \multicolumn{2}{c}{100}	 & 0.19559	     & 0.27549	        & 0.31023           & 0.33378			     & 0.35264\\
	& \simPY	    & Yes		    & No		  & 2	       & \multicolumn{2}{c}{100}	 & 0.19559	     & 0.27549	        & 0.31023           & 0.33378			     & 0.35264\\


	%\hline
        \cmidrule(r){1-12}
        

        \multirow{6}{*}{\TptCF}
        & \multicolumn{3}{c}{\#sim\_pats}  &  \multicolumn{3}{c}{term\_sim\_threshold}  & \small{HR@$1$} & \small{HR@$2$}  & \small{HR@$3$}  & \small{HR@$4$} & \small{HR@$5$} \\
        \cmidrule(r){2-12} 
        % 
	& \multicolumn{3}{c}{2,200}        &  \multicolumn{3}{c}{1.0}                   & 0.28533          & 0.37321           & 0.40079           & 0.42062          & 0.43470\\
	& \multicolumn{3}{c}{2,200}        &  \multicolumn{3}{c}{1.0}                   & 0.28533          & 0.37321           & 0.40079           & 0.42062          & 0.43470\\
	& \multicolumn{3}{c}{2,600}	   &  \multicolumn{3}{c}{0.6}			& 0.28309	   & 0.37247	       & 0.40213	   & 0.42196	      & 0.43709\\
	& \multicolumn{3}{c}{2,000}	   &  \multicolumn{3}{c}{0.3}			& 0.27668	   & 0.36576	       & 0.39930	   & 0.42405	      & 0.43798\\
	& \multicolumn{3}{c}{2,600}	   &  \multicolumn{3}{c}{0.3}			& 0.27706          & 0.36628           & 0.39945           & 0.42397          & 0.43828\\
                                                                                                                                                    

	%
        \cmidrule(r){1-12}
        \multirow{6}{*}{\method\_\ypCF}
	& Identification  & \physician\_self\_ref & \patient\_self\_ref & \#sim\_phy & \#sim\_pat & $\alpha$  & \small{HR@$1$}  & \small{HR@$2$} & \small{HR@$3$}  & \small{HR@$4$}  & \small{HR@$5$}    \\

        \cmidrule(r){2-12}
	& \simYP          & No                   & No                  & 1          & 1           & 0.1       & 0.30605           & 0.40668          & 0.45110           & 0.47801           & 0.50104\\
	& \simYP          & No                   & No                  & 1          & 2           & 0.1       & 0.30359           & 0.40720          & 0.45036           & 0.47786           & 0.50209\\
	& \simYP          & No                   & No                  & 1          & 100	  & 0.1	      & 0.30389		  & 0.40534          & 0.45170	         & 0.48315	     & 0.50939\\
	& \simYP          & No                   & No                  & 1          & 100	  & 0.1	      & 0.30389		  & 0.40534          & 0.45170	         & 0.48315	     & 0.50939\\
	& \simYP          & No                   & No                  & 1          & 100	  & 0.1	      & 0.30389		  & 0.40534          & 0.45170	         & 0.48315	     & 0.50939\\

	\cmidrule(r){1-12}
	\multirow{6}{*}{\method\_\TptCF}
	& \multicolumn{3}{c}{\#sim\_pats}  &  \multicolumn{2}{c}{term\_sim\_threshold} & $\alpha$  & \small{HR@$1$} & \small{HR@$2$}  & \small{HR@$3$}  & \small{HR@$4$} & \small{HR@$5$} \\
	\cmidrule(r){2-12}
	& \multicolumn{3}{c}{1}            &  \multicolumn{2}{c}{0.3}                  & 0.1       & 0.32841          & 0.42211           & 0.46005           & 0.48614  & 0.50857\\
	& \multicolumn{3}{c}{1}		   &  \multicolumn{2}{c}{0.1}		       & 0.1	   & 0.32834	      & 0.42270		  & 0.46035	      & 0.48830  & 0.50939\\
	& \multicolumn{3}{c}{1}            &  \multicolumn{2}{c}{0.1}                  & 0.1       & 0.32834          & 0.42270           & 0.46035           & 0.48830
& 0.50939\\
	& \multicolumn{3}{c}{1}            &  \multicolumn{2}{c}{0.1}                  & 0.1       & 0.32834          & 0.42270           & 0.46035           & 0.48830
& 0.50939\\
	& \multicolumn{3}{c}{5}		   &  \multicolumn{2}{c}{0.1}		       & 0.1	   & 0.32491	      & 0.42054		  & 0.45953	      & 0.48748  & 0.51044\\


        \bottomrule%\bottomrule
%      \hline\hline
      \end{tabular}
\begin{comment}
      \begin{tablenotes}
       \begin{scriptsize}
          \setlength\labelsep{0pt}
        \item 
          \par
        \end{scriptsize}
      \end{tablenotes}
\end{comment}
  \end{threeparttable}
  \end{small}
  } %end tbl
%\vspace{-10pt}
\end{table*}


